Human Motion Transfer from Poses in the Wild

In this paper, we tackle the problem of human motion transfer, where we synthesize novel motion video for a target person that imitates the movement from a reference video. It is a video-to-video translation task in which the estimated poses are used to bridge two domains. Despite substantial progress on the topic, there exist several problems with the previous methods. First, there is a domain gap between training and testing pose sequences--the model is tested on poses it has not seen during training, such as difficult dancing moves. Furthermore, pose detection errors are inevitable, making the job of the generator harder. Finally, generating realistic pixels from sparse poses is challenging in a single step. To address these challenges, we introduce a novel pose-to-video translation framework for generating high-quality videos that are temporally coherent even for in-the-wild pose sequences unseen during training. We propose a pose augmentation method to minimize the training-test gap, a unified paired and unpaired learning strategy to improve the robustness to detection errors, and two-stage network architecture to achieve superior texture quality. To further boost research on the topic, we build two human motion datasets. Finally, we show the superiority of our approach over the state-of-the-art studies through extensive experiments and evaluations on different datasets.

==> 3_data_processing.tex <==
\begin{figure}[t]
\begin{center}
\includegraphics[width=1\columnwidth]{3_data_processing.jpg}
\caption{\textbf{Training data preparation}. (a) One example frame captured in front of the green screen. (b) Extract the pose skeleton and remove the background, the pose information is further used to calculate the cropping region around the person. (c) Crop the foreground and fill the background with solid green color. (c) Perform data augmentation on the poses, such as elongating or shortening both arms as indicates by the arrows.}
\label{fig:dp}
\end{center}
\end{figure}



==> 4_comparisons.tex <==
\begin{table}[t]
\centering
\caption{\textbf{Objective comparisons} on the Target-Vali dataset.}
\begin{tabular}{C{2.5cm} | C{2.2cm}|  C{2.2cm} }
\hline
&SSIM $\uparrow$ &  FID $\downarrow$  \\ \hline\hline
vid2vid & 0.9518  &7.5214\\ 
ours& 0.9666  & 5.9453 \\ \hline
\end{tabular}
\label{tab:SOTA}
\end{table}

